On concentration in vortex sheets

The question of energy concentration in approximate solution sequences $u^\epsilon$, as $\epsilon \to 0$, of the two-dimensional incompressible Euler equations with vortex-sheet initial data is revisited. Building on a novel identity for the structure function in terms of vorticity, the vorticity maximal function is proposed as a quantitative tool to detect concentration effects in approximate solution sequences. This tool is applied to numerical experiments based on the vortex-blob method, where vortex sheet initial data without distinguished sign are considered, as introduced in \emph{[R.~Krasny, J. Fluid Mech. \textbf{167}:65-93 (1986)]}. Numerical evidence suggests that no energy concentration appears in the limit of zero blob-regularization $\epsilon \to 0$, for the considered initial data.

==> preamble.tex <==
% useful packages
\usepackage{amsthm,amssymb}
\usepackage{mathtools,thmtools}
\usepackage{bm,esint}
\usepackage{color}
\usepackage{float,graphicx,subcaption}
\usepackage{cleveref}
\usepackage{cancel}

% useful short-hand definitions
% some commands
\DeclareMathOperator*{\esssup}{ess\,sup}

% explanation for equation
\renewcommand{\vec}{\bm}
\newcommand{\explain}[2]{\overset{\mathclap{\underset{\downarrow}{#2}}}{#1}}
%
\newcommand{\loc}{{\mathrm{loc}}}
\newcommand{\dirac}{\delta}
\newcommand{\slot}{{\,\cdot\,}}
\newcommand{\dom}{{\R^2}}
%
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\defeq}{{:=}}
\renewcommand{\d}{{\mathrm{d}}}
\newcommand{\intF}{{\int_{L^p}}}
\newcommand{\intav}{{\hspace{5pt}-\hspace{-10pt}\int}}
\newcommand{\weaklyto}{{\rightharpoonup}}
\newcommand{\weakstarto}{\overset{\ast}{\weaklyto}}
% mathbb
\newcommand{\T}{\mathbb{T}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
%
\renewcommand{\div}{{\mathrm{div}}}
\newcommand{\curl}{{\mathrm{curl}}}
\newcommand{\Lip}{\mathrm{Lip}}

%
\renewcommand{\P}{{\mathcal{P}}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\eps}{\epsilon}
\newcommand{\e}{\eps}

\newcommand{\define}{\textbf}
\newcommand{\Prob}{\mathcal{P}}
\newcommand{\U}{U}
\newcommand{\ip}[2]{{\langle #1, #2 \rangle}}
\newcommand{\intavg}{\fint}
\newcommand{\Lp}{{\mathfrak{L}}}

%
\newcommand{\uhat}{{\widehat{\vec{u}}}}
\newcommand{\u}{{\vec{u}}}
